Smoothed Analysis of Online and Differentially Private Learning

Practical and pervasive needs for robustness and privacy in algorithms have inspired the design of online adversarial and differentially private learning algorithms. The primary quantity that characterizes learnability in these settings is the Littlestone dimension of the class of hypotheses [Ben-David et al., 2009, Alon et al., 2019]. This characterization is often interpreted as an impossibility result because classes such as linear thresholds and neural networks have infinite Littlestone dimension. In this paper, we apply the framework of smoothed analysis [Spielman and Teng, 2004], in which adversarially chosen inputs are perturbed slightly by nature. We show that fundamentally stronger regret and error guarantees are possible with smoothed adversaries than with worst-case adversaries. In particular, we obtain regret and privacy error bounds that depend only on the VC dimension and the bracketing number of a hypothesis class, and on the magnitudes of the perturbations.

==> app_example.tex <==
\section{Lack of Uniform Convergence in Smooth Adaptive}

\subsection{Adaptive Adversary} \label{subsec:ada}
As we observed in the previous section (Lemma~\ref{lem:non-ada-gen}),
any hypothesis class $\G$ with bounded VC dimension demonstrates
uniform convergence on any non-adaptive sequence of distributions
$\bP$, regardless of the smoothness of $\bP$ or other properties of
$\G$. 
The next example demonstrates that this property fails to hold with
adaptive adversaries.
%In the case of an adaptive sequence of distributions, however, we show that %such a property fails to hold.

\begin{example}
Let $\X = [0,1]$ and $\G = \{g_b(x) = \one(x\geq b) \mid \forall b\in[0,1] \}$ be the set of one-dimensional thresholds. Let $\td$ be an adaptive sequence of distributions, such that $\P_1$ is a uniform distribution over $[0,\frac 14]\cup [\frac 34, 1]$ and $\P_2 = \dots = \P_T$ all are  the uniform distribution on $[0,\frac 14]$ if $x_1\in[0,1/4]$, and otherwise, are the uniform distribution on $[\frac 34, 1]$. In this case, we do not achieve concentration for any value of $T$, as
\[
\frac 1T \sum_{t=1}^T g_{0.5}(x_t) = \begin{cases} 0 & \text{w.p. $1/2$}\\ 1 & \text{w.p. $1/2$} \end{cases} \qquad and \qquad  \E_{\vec x \sim \td} \left[  \frac 1T \sum_{t=1}^T g_{0.5}(x_t) \right] = \frac 12.
\]
\end{example}
An even more troubling aspect of the above example is that $\td$ is $\frac 14$-smooth and $\G$ has a VC dimension of $1$. So, smoothness of an adaptive distribution is not sufficient for obtaining uniform convergence over $\G$, even if $\G$ has a small VC dimension.


At a high level, one of the challenging aspects of the above example
is that $\{ x \mid g_{0.5}(x) = 1\}$ is relatively large.  This allows
an adaptive adversary to create a smooth $\td$ where the supports of
$\P_2, \dots, \P_T$ are all within the set $\{x \mid g(x) =1\}$ if
some constant-probability event takes place in the first round, and
otherwise choosing smooth $\P_2, \dots, \P_T$ whose supports are
within the set $\{x \mid g(x) = 0\}$.  
A key observation is that the hypotheses that we really care
about are those in $\A$, each of which is the symmetric
difference of two similar hypotheses.  That is, $\Pr_\U[a(x) = 1]$ is
small for all $a \in \A$.  As we'll see, this additional property is
sufficient to obtain good regret bounds in the adaptive case.

